Determination of CP-violating $HZZ$ interaction with polarised beams at the ILC

We study possible CP-violation effects of the 125 GeV Higgs to $Z$ boson coupling at the 250 GeV ILC with transverse and longitudinal beam polarisation via the process $e^+ e^- \rightarrow HZ \rightarrow H \mu^-\mu^+$. We explore the azimuthal angular distribution of the muon pair from the $Z$ boson decay, and constructe CP-odd observables sensitive to CP-violation effects, where we derived this observable both by analytical calculations and by $\mathtt{Whizard}$ simulations. Particularly, we can construct two CP-odd observables with the help of transversely-polarised initial beams and improve the statistical significance of CP-violation effects by combining two measurements. We defined the asymmetries between the signal regions with different signs of the CP-odd observables, and determine the CP-violation effect by comparing with the SM 95% C.L. upper bound. In this paper, we setup a scenario which assumes that the total cross-section is always fixed while CP-violation is varying, and such a scenario helps us to determine the intrinsic CP-mixing angle limit around $|\xi_{CP}|\sim 0.03$ with (90%, 40%) polarised electron-positron beams and 5 ab$^{-1}$ integrated luminosity. In addition, we determine the CP-odd coupling limit $|\widetilde{c}_{HZZ}|\sim 0.01$ as well, where we suppose that the SM tree-level cross-section is fixed and the CP-violation is the varying additional contribution. Comparing with the analysis with unpolarised beams, the sensitivity to the CP-violation effect can be improved by transverse or longitudinal polarisation.

==> backup.tex <==
\section{The analytical result of cross section}
\label{sec:xseehmumu}
In order to calculate the cross section of $e^-(p_1) e^+(p_2) \rightarrow Z(p_3) H(p_4) \rightarrow \mu^-(p_5)\mu^+(p_6)$ process, we applied the narrow width approximation, and calculate the Higgs strahlung and $Z$ decay separately.

For the SM Higgs strahlung $e^-(p_1,\lambda_r) e^+(p_2, \lambda_u) \rightarrow Z(p_3, \lambda^i) H$, the scattering amplitude with the spin indices of the initial electron, positron and the $Z$ boson is given by:
{\fontsize{11}{11}\selectfont
\begin{equation}
    \mathcal{M}_{\lambda_r \lambda_s}^{\lambda^i}=\bar{v}(p_2,\lambda_u)\Big[ i\frac{g^2 m_Z}{2 c_W^2 }\frac{-\eta_{\mu\nu}+\frac{k_\mu k_\nu}{m_Z^2}}{k^2-m_Z^2}\gamma^\mu(c_V+c_A\gamma_5) {\varepsilon^*}^\nu(p_3, \lambda^i)\Big] u(p_1, \lambda_r)
\end{equation}}

After applying the Bouchiat-Michel formula of Eq.~\eqref{eq:boumi_uu} and polarization matrix of Eq.~\eqref{eq:polmat}, the result of the scattering amplitude square is given by:
\begin{equation}
       \rho^{ii'}= (1-P^3_-P^3_+)A + (P^3_- - P^3_+)B + \sum^{1,2}_{mn}P^m_- P^n_+ C_{mn}
\end{equation}
For the SM, the unpolarized part is:
\begin{multline}
    A_\text{SM} = \frac{g^4m_Z^2}{4c_W^2(s-m_Z^2)}\Big( (c_V^2 +c_A^2)[(\varepsilon^i\cdot p_2)({\varepsilon^*}^{i'}\cdot p_1)+(\varepsilon^i\cdot p_1)({\varepsilon^*}^{i'}\cdot p_2)-(\varepsilon^i\cdot {\varepsilon^*}^{i'})(p_2\cdot p_1)]\\-{i}2c_Vc_A\epsilon_{\alpha\mu\beta\nu}{\varepsilon^i}^\alpha{\varepsilon^\beta}^{i'} {p_1}^\mu {p_2}^\nu\Big),
\end{multline}
and the longitudinally polarized part is 
\begin{multline}
    B_\text{SM} = \frac{g^4m_Z^2}{4c_W^2(s-m_Z^2)}\Big( 2c_V c_A[(\varepsilon^i\cdot p_2)({\varepsilon^*}^{i'}\cdot p_1)+(\varepsilon^i\cdot p_1)({\varepsilon^*}^{i'}\cdot p_2)-(\varepsilon^i\cdot {\varepsilon^*}^{i'})(p_2\cdot p_1)]\\-{i}(c_V^2+c_A^2)\epsilon_{\alpha\mu\beta\nu}{\varepsilon^i}^\alpha{\varepsilon^\beta}^{i'} {p_1}^\mu {p_2}^\nu\Big),
\end{multline}
as well as the transversely polarized part
{\small
\begin{multline}
    C^{mn}_\text{SM}=\frac{g^4m_Z^2(c_A^2-c_V^2)}{4c_W^2(s-m_Z^2)}\Big(  (s_-^m\cdot s_+^n)[(\varepsilon^i\cdot p_1)({\varepsilon^*}^{i'}\cdot p_2)+(\varepsilon^i\cdot p_2)({\varepsilon^*}^{i'}\cdot p_1)-(\varepsilon^i\cdot{\varepsilon^*}^{i'})(p_1\cdot p_2)] \\+(p_1\cdot p_2)[(\varepsilon^i\cdot s_+^n)({\varepsilon^*}^{i'}\cdot s_-^m)+(\varepsilon^i\cdot s_-^m)({\varepsilon^*}^{i'}\cdot s_+^n)] \Big).
\end{multline}}

For the $Z(p_3)\rightarrow \mu^-(p_5) \mu^+(p_6)$ decay, we have the amplitude:
\begin{equation}
    \mathcal{M}^i = \frac{ig}{2c_W}{\varepsilon^\lambda}^i  \bar{u}(p_5)\gamma_\lambda (c_V+c_A\gamma_5)v(p_6)
\end{equation}
\begin{multline}
    \rho^{i i'}_D = \frac{g^2}{c_W^2}\Big( (c_V^2+c_A^2)[(\varepsilon^i\cdot p_5)({\varepsilon^*}^{i'}\cdot p_6) + (\varepsilon^i\cdot p_6)({\varepsilon^*}^{i'}\cdot p_5)+\delta^{ii'}(p_5\cdot p_6)] \\-i2c_V c_A \epsilon_{\alpha\mu\beta\nu}{\varepsilon^i}^\alpha {{\varepsilon^*}^{i'}}^\beta p^\mu_5 p_6^\nu \Big)
\end{multline}

By using the narrow width approximation of Eq.~\eqref{eq:narrowxs}, the full scattering amplitude square is given by:
{%\fontsize{12}{12}\selectfont
\begin{equation}
    \begin{split}
&|M|^2 = \frac{g^6 m_Z}{4c_W^6(s-m_Z^2)^2\Gamma_Z} \Big\{    (1-P_-^3 P_+^3)\Bigl[ 2(c_V^2+c_A^2)^2\Big(\frac{(p_1\cdot p_3)(p_2\cdot p_3)}{m_Z^2}(p_5\cdot p_6) \\&\qquad- \frac{(p_3\cdot p_5)^2}{m_Z^2}(p_1\cdot p_2)-2[\frac{(p_1\cdot p_3)(p_3\cdot p_5)}{m_Z^2}-p_1\cdot p_5][\frac{(p_2\cdot p_3)(p_3\cdot p_5)}{m_Z^2}-p_2\cdot p_5]\Big)\\&\qquad-24c_V^2 c_A^2[(p_1\cdot p_5)(p_2\cdot p_6)-(p_1\cdot p_6)(p_2\cdot p_6)] \Bigr]\\
&+(P^3_- -P^3_+)2c_V c_A\Bigl[    (c_V^2+c_A^2)\Big(\frac{(p_1\cdot p_3)(p_2\cdot p_3)}{m_Z^2}(p_5\cdot p_6) - \frac{(p_3\cdot p_5)^2}{m_Z^2}(p_1\cdot p_2)\\
&\qquad-2[\frac{(p_1\cdot p_3)(p_3\cdot p_5)}{m_Z^2}-p_1\cdot p_5][\frac{(p_2\cdot p_3)(p_3\cdot p_5)}{m_Z^2}-p_2\cdot p_5]\\&\qquad-6[(p_1\cdot p_5)(p_2\cdot p_6)-(p_1\cdot p_6)(p_2\cdot p_6)]\Big)\Bigr]\\
&-\sum_{m,n}P^m_-P^n_+ \Bigl[(c_V^4-c_A^4)\big[(s_-^m\cdot s_+^n)\Bigl(\frac{(p_1\cdot p_3)(p_2\cdot p_3)}{m_Z^2}(p_5\cdot p_6) - \frac{(p_3\cdot p_5)^2}{m_Z^2}(p_1\cdot p_2)\\
&\qquad-2[\frac{(p_1\cdot p_3)(p_3\cdot p_5)}{m_Z^2}-p_1\cdot p_5][\frac{(p_2\cdot p_3)(p_3\cdot p_5)}{m_Z^2}-p_2\cdot p_5]\Bigr)\\&\qquad+2(p_1\cdot p_2)\Bigl((p_5\cdot p_6)(\frac{(p_3\cdot s_+^n)(p_3\cdot s_-^m)}{m_Z^2}-s_+^n\cdot s_-^m)\\
&\qquad-2(\frac{(p_3\cdot s_+^n)(p_3\cdot p_5)}{m_Z^2}-p_5\cdot s_+^n)(\frac{(p_3\cdot s_-^m)(p_3\cdot p_5)}{m_Z^2}-p_5\cdot s_-^m)\Bigr)\big]  \Bigr]
\Big\}
\end{split}
\end{equation}}


For the case with the BSM $\mathcal{CP}$-odd contribution, the result of the full scattering amplitude square still takes the form of Eq.~\eqref{eq:matpol}, which can be separated into the three parts as well. Therefore, we have:
\begin{multline}
    |\mathcal{M}|^2= (1-P^3_-P^3_+)( c_\alpha^2 \kappa^2_\text{SM} A_\text{SM} + s_\alpha c_\alpha\kappa_\text{SM}\Tilde{\kappa}_{HZZ} {A}_\text{CP-odd} +s_\alpha^2 \Tilde{\kappa}_{HZZ}^2 \tilde{{A}}_\text{CP-even}) \\
    + (P^3_- - P^3_+)( c_\alpha^2 \kappa^2_\text{SM} B_\text{SM} + s_\alpha c_\alpha\kappa_\text{SM}\Tilde{\kappa}_{HZZ} B_{\mathrm{CP-odd}} +s_\alpha^2 \Tilde{\kappa}_{HZZ}^2 \tilde{B}_{\mathrm{CP-even}}) \\
    + \sum^{1,2}_{mn}P^m_- P^n_+ ( c_\alpha^2 \kappa^2_\text{SM} C^{mn}_\text{SM} + s_\alpha c_\alpha\kappa_\text{SM}\Tilde{\kappa}_{HZZ} C^{mn}_{\mathrm{CP-odd}} +s_\alpha^2 \Tilde{\kappa}_{HZZ}^2 C^{mn}_{\mathrm{CP-even}})
\end{multline}
where for the $\mathcal{CP}$-odd part, we have:
\begin{multline}
     A_{\mathrm{CP-odd}} = - \frac{g^6 \epsilon_{\alpha\beta\mu\nu}p_1^\alpha p_2^\beta p_3^\mu p_5^\nu}{c_W^6(s-m_Z^2)^2m_Z^3\Gamma_Z}\Big[ 2(c_V^2 + c_A^2)^2(p_3\cdot p_5)(p_1 -p_2)\cdot p_3 \\+m_Z^2 (2c_V^2c_A^2(p_1 + p_2)\cdot p_3-(c_V^2 + c_A^2)^2 (p_1 -p_2 )\cdot p_5)\Big],
     \label{eq:cpmixa}
\end{multline}
\begin{multline}
     B_{\mathrm{CP-odd}} = \frac{g^6 \epsilon_{\alpha\beta\mu\nu}p_1^\alpha p_2^\beta p_3^\mu p_5^\nu}{c_W^6(s-m_Z^2)^2m_Z^3\Gamma_Z}c_A c_V(c_A^2 + c_V^2)[2(p_3\cdot p_5) (p_1-p_2)\cdot p_3\\+m_Z^2 ((p_1+p_2)\cdot p_3 -2 (p_1-p_2)\cdot p_5)]
\end{multline}
and
\begin{multline}
     C^{mn}_{\mathrm{CP-odd}} = -\frac{g^6(c_A^4 - c_V^4)}{2 c_W^6(s-m_Z^2)^2m_Z^3\Gamma_Z}\Big[ 2(s_+^n\cdot s_-^m)((p_3\cdot p_5 )(p_1-p_2)\cdot p_3\\-m_Z^2 (p_1-p_2)\cdot p_5)\epsilon_{\alpha\beta\mu\nu}p_1^\alpha p_2^\beta p_3^\mu p_5^\nu \\
     + s[\epsilon_{\alpha\beta\mu\nu}(p_1+p_2)^\alpha p_3^\beta p_5^\mu {s_-^m}^\nu((p_3\cdot p_5)(s_+^n\cdot p_3)-(s_+^n\cdot p_5)m_Z^2)  \\+ \epsilon_{\alpha\beta\mu\nu}(p_1+p_2)^\alpha p_3^\beta p_5^\mu {s_+^n}^\nu((p_3\cdot p_5)(s_-^m\cdot p_3)-(s_-^m\cdot p_5)m_Z^2)     ]  \Big]
     \label{eq:cpmixc}
\end{multline}

Lastly, the part of the CP-odd contributions are:
{\small
\begin{multline}
\tilde{A}_{\mathrm{CP-even}} = \frac{g^6}{8m_Z^3 c_W^6 (s-m_Z^2)^2\Gamma_Z}\Big[-8(c_A^2 + c_V^2)((p_1\cdot p_5) (p_2\cdot p_3) - (p_1\cdot p_3) (p_2\cdot p_5))^2\\
    + 2s (p_3\cdot p_5) ((c_A^4+c_V^4)[((p_1\cdot p_3))^2 + ((p_2\cdot p_3))^2-2((p_1+p_2)\cdot p_3)((p_1-p_2)\cdot p_5)]\\
+2c_A^2 c_V^2[3((p_1\cdot p_3))^2 - ((p_2\cdot p_3))^2-2((p_1-p_2)\cdot p_3)((p_1-p_2)\cdot p_5)])
    \\-   s m_Z^2[-2(c_V^2 +c_A^2)^2((p_1-p_2)\cdot p_5)^2  -8c_A^2c_V^2 ((p_1-p_2)\cdot p_5)((p_1-p_2)\cdot p_3) ]\\ -s^2 m_Z^2 (c_A^2 + c_V^2)^2(p_3\cdot p_5)\Big]
\end{multline}}
\begin{multline}
 \tilde{B}_{\mathrm{CP-even}}=\frac{g^6 c_A c_V (c_A^2 + c_V^2)}{8m_Z^3 c_W^6 (s-m_Z^2)^2\Gamma_Z}   \Bigl[8((p_1\cdot p_5) (p_2\cdot p_3) - (p_1\cdot p_3) (p_2\cdot p_5))^2 \\
  + s^2 m_Z^2 (p_3\cdot p_5) -  4s (p_3\cdot p_5)[(p_1\cdot p_3)^2- ((p_1-p_2)\cdot p_3)((p_1-p_2)\cdot p_5)]\\
 +2s m_Z^2 [((p_1-p_2)\cdot p_3)((p_1+p_2)\cdot p_5) - ((p_1\cdot p_5) - (p_2\cdot p_5))]\Bigr]
\end{multline}
and
\begin{multline}
 \tilde{C}^{mn}_{\mathrm{CP-even}}=-\frac{g^6(c_A^4 - c_V^4)}{8m_Z^3 c_W^6 (s-m_Z^2)^2\Gamma_Z}   \Big[8 (s_-^m\cdot s_+^n) [(p_1\cdot p_3)(p_2\cdot p_5) -(p_2\cdot p_3)(p_1\cdot p_5)]^2\\
     + 2s \Bigl((s_-^m\cdot s_+^n) (p_3\cdot p_5) [ (p_1\cdot p_3) (p_2\cdot p_3) - (p_1\cdot p_5) (p_1\cdot p_3) - (p_2\cdot p_3) (p_2\cdot p_5)\\ - 3 (p_1\cdot p_5) (p_2\cdot p_3)  -3 (p_1\cdot p_3) (p_2\cdot p_5)  ]\\
+ ((p_1  + p_2)\cdot p_3) ((p_1+p_2)\cdot p_5) ((s_-^m\cdot p_5) (s_+^n\cdot p_3)+(s_-^m\cdot p_3) (s_+^n\cdot p_5))\\
- ((p_1+ p_2)\cdot p_5)^2 (s_-^m\cdot p_3) (s_+^n\cdot p_3)- ((p_1+p_2)\cdot p_3)^2 (s_+^n\cdot p_5) (s_-^m\cdot p_5) 
    \Bigr)\\
+ s m_Z^2 [2(s_-^m\cdot s_+^n)(((p_1 + p_2)\cdot p_5 )^2 + 4 (p_1\cdot p_5) (p_2\cdot p_5))]\\
    +s^2 (p_3\cdot p_5) [(s_-^m\cdot p_3)(s_+^n\cdot p_3)-2(s_-^m\cdot p_5)(s_+^n\cdot p_3)-(s_+^n\cdot p_5)(s_-^m\cdot p_3) \\+ 2(p_3\cdot p_5)(s_-^m\cdot s_+^n)]
 \Big]
 \Big]
\end{multline}

and the total cross section can be the above result applied into the Eq.~\eqref{eq:xstot}, and obtained by the numerical integration.

\section{The phase space}
\label{sec:dlips}
As we know, one can eventually obtain the cross section of $e^+ e^- \rightarrow H \mu^+ \mu^-$ process by integrating over the three-body phase space. However, one of the degrees of freedom can be integrated out by applying the narrow width approximation, and there are only four degrees of freedom in the final phase space. In this case, the Lorentz invariant phase space is given by:
\begin{equation}
    dQ=\frac{1}{(2\pi)^4}\frac{d\Omega_H d\Omega_{\mu^-}}{16\sqrt{s}}\frac{|p_H^f| |p_{\mu^-}^f|}{|\Vec{p}_H+\Vec{p}_{\mu^-}|+|p_{\mu^-}^f|+|p_H^f| \cos\theta_{H\mu}}=Q~d\Omega_H d\Omega_{\mu^-}
    \label{eq:dlips}
\end{equation}
where:
\begin{align}
    &|p_H^f| = \frac{1}{2\sqrt{s}}\sqrt{(s-(m_H+m_Z)^2)(s-(m_H-m_Z)^2)}\\
    &|p_{\mu^-}^f| = \frac{m_Z^2}{2\sqrt{|p_H^f|^2 + m_Z^2} + |p_H^f|\cos\theta_{H\mu}}
\end{align}
The term $\cos\theta_{H\mu}$ indicate the projection of the muon momentum on the Higgs momentum.

In particular, we can evaluate the phase space in the center of mass frame.
If the electron and positron beams are transversely polarized, their spin vector $\Vec{s}_{e^\pm}$ would be perpendicular to their momentum $\Vec{p}_{e^\pm}$. In this case, we can define a coordinate system by using the spin vector and momentum of electron beams $\Vec{s}_{e^-},~\Vec{p}_{e^-}$, where the momentum of final state particles are shown in Fig.~\ref{fig:eehmumu_coord}. Consequently, the projection $\cos\theta_{H\mu}$ can be expressed as :
\begin{equation}
    \begin{split}
        \cos\theta_{H\mu} = &-\sin\theta_H\cos\phi_H \sin\theta_{\mu^-} \cos\phi_{\mu^-}-\sin\theta_H\sin\phi_H \sin\theta_{\mu^-}\sin\phi_{\mu^-}\\
        &-\cos\theta_H \cos\theta_{\mu^-}.
    \end{split}
\end{equation}

\section{Matching relations between different interpretations}
\label{sec:matching}
\subsection*{Effective $\cp$-odd fraction}
In order to estimate the $\cp$-odd contribution on the total cross-section, one can define a effective $\cp$-odd fraction $f^{HZZ}_{CP}$ refer to \cite{Dawson:2013bba}
\begin{equation}
    f^{HZZ}_{CP} = \frac{|\widetilde{c}_{HZZ}|^2 \widetilde{\sigma}_{HZZ}}{\sigma_\mathrm{tot}}.
    \label{eq:fcp}
\end{equation}
where $\widetilde{\sigma}_{HZZ}$ is the cross-section obtained by setting $c_\mathrm{SM}=c_{HZZ}=0$ and $\widetilde{c}_{HZZ}=1$. If we assume that the $\cp$-odd term $\widetilde{c}_{HZZ}$ is the unique BSM contribution, and the SM tree-level contribution stays invariant, the effective $\cp$-odd fraction is given by%only obtained from the amplitude $\epsilon_{\mu\nu\alpha\beta}\mathcal{M}^{\mu\nu}p^\alpha p^\beta$.
\begin{equation}
    f^{HZZ}_{CP} = \frac{1}{1 + \frac{\sigma_\mathrm{SM}}{|\widetilde{c}_{HZZ}|^2\widetilde{\sigma}_{HZZ}}} = \frac{1}{1+\frac{\sigma_\mathrm{SM}}{|a_3|^2\sigma_3} }
    \label{eq:fcp2}
\end{equation}
However, the effective $\cp$-odd fraction is also depending on the concrete processes. Particularly, we have the numbers for the following processes
\begin{gather}
    \frac{\sigma_3}{\sigma_\mathrm{SM}}[pp\rightarrow H\rightarrow 4\ell (13~\mathrm{TeV})] \sim 0.153, \\~~\frac{\widetilde{\sigma}_{HZZ}}{\sigma_\mathrm{SM}}[e^+ e^-\rightarrow H \mu^+ \mu^- (250~\mathrm{GeV})] \sim 0.503.
\end{gather}
Furthermore, one can also define a effective $\cp$-mixing angle $\psi_\cp$ by using the effective $\cp$-odd fraction, which is given by:
\begin{equation}
    \sin^2\psi_\cp = f^{HZZ}_{CP} = \sin^2\xi_\cp\frac{ \tilde{\kappa}^2_{HZZ}\tilde{\sigma}_{HZZ}}{\sigma_\mathrm{tot}}
\end{equation}

\subsection*{$\cp$-odd couplings}

%  is defined by the following effective Lagrangian
% \begin{equation}
%     \mathcal{L}_\mathrm{eff}  = \frac{g}{2m_W} a_3 Z_{\mu\nu}Z^{\mu\nu}H
% \end{equation}
The coupling $a_3$ in Eq.~\eqref{eq:fcp2} can be converted to another interpretation of $\cp$-odd coupling by the following relation \cite{CMS:2021nnc}
\begin{equation}
    \Tilde{c}_{ZZ} = -\frac{\sin^2\theta_W\cos^2\theta_W}{2\pi\alpha} a_3
\end{equation}
where the coupling $\Tilde{c}_{ZZ}$ is defined by the following effective Lagrangian in Eq.(21) of \cite{Cepeda:2019klc}
\begin{equation}
    \mathcal{L}_\mathrm{eff} = \frac{g_1^2+g_2^2}{4}\Tilde{c}_{ZZ} \frac{H}{v}Z_{\mu\nu}\Tilde{Z}^{\mu\nu}
\end{equation}
Therefore, we have the matching relation
\begin{equation}
    \widetilde{c}_{HZZ}=\frac{g_1^2+g_2^2}{4}\Tilde{c}_{ZZ} = \frac{m_Z^2}{v^2} \Tilde{c}_{ZZ}
\end{equation}

By using the matching relation, we can convert our results to the $\tilde{c}_{ZZ}$ interpretation, and the summary table of $\tilde{c}_{ZZ}$ is given by Tab.~\ref{tab:comp_exp_czz}.
\begin{table}[h]
    \centering
    \resizebox{\linewidth}{!}{\begin{tabular}{c|ccccccc}
    \hline
       Experiments&  ATLAS\cite{ATLAS:2023mqy}& CMS\cite{CMS:2021nnc}& HL-LHC\cite{Cepeda:2019klc}& CEPC\cite{Sha:2022bkt}& CLIC\cite{Karadeniz:2019upm}& CLIC \cite{Vukasinovic:2023jxd}& ILC\\
       Processes& $H\rightarrow 4\ell$& $H\rightarrow 4\ell$& $H\rightarrow 4\ell$& $ H Z$&  $W$-fusion& $Z$-fusion &$ H Z,~Z\rightarrow \mu^+\mu^-$\\
       $\sqrt{s}$ [GeV]&  13000&  13000& 14000& 240& 3000& 1000& 250\\
       Luminosity~[fb$^{-1}$]&  139& 137& 3000& 5600& 5000& 1000& 5000\\
       % & & & & &  & $(P^L_{-},P^L_{+})$\\
       $(|P_{-}|,|P_{+}|)$& & & & & & $(100\%, 100\%)$& $(90\%, 40\%)$\\
       \hline
       $\tilde{c}_{ZZ}$ &&&&&&\\
       95\% C.L. (2$\sigma$)limit&   [-1.2, 1.75]& [-0.66, 0.51]& [-0.66, 0.66]& [-0.12, 0.12]& [-0.24, 0.24]& [-0.12, 0.12]&  [-0.08, 0.07] \\
       \hline
    \end{tabular}}
    \caption{Summary of the limits of $\tilde{c}_{ZZ}$ at 95\% C.L., where the results are obtained from both current LHC measurements and future colliders analysis, including HL-LHC, CEPC, ILC and CLIC.}
    \label{tab:comp_exp_czz}
\end{table}
